Transductive Learning for Abstractive News Summarization

Pre-trained and fine-tuned news summarizers are expected to generalize to news articles unseen in the fine-tuning (training) phase. However, these articles often contain specifics, such as new events and people, a summarizer could not learn about in training. This applies to scenarios such as a news publisher training a summarizer on dated news and summarizing incoming recent news. In this work, we explore the first application of transductive learning to summarization where we further fine-tune models on test set inputs. Specifically, we construct pseudo summaries from salient article sentences and input randomly masked articles. Moreover, this approach is also beneficial in the fine-tuning phase, where we jointly predict extractive pseudo references and abstractive gold summaries in the training set. We show that our approach yields state-of-the-art results on CNN/DM and NYT datasets, improving ROUGE-L by 1.05 and 0.74, respectively. Importantly, our approach does not require any changes of the original architecture. Moreover, we show the benefits of transduction from dated to more recent CNN news. Finally, through human and automatic evaluation, we demonstrate improvements in summary abstractiveness and coherence.

==> content/background.tex <==
\section{Background}

In this section, we review related modelling aspects. And in Sec. \ref{sec:approach}, we dive into details of our approach. 


\subsection{Pre-training and Fine-tuning}
\label{sec:pre_fine_tune}

Unsupervised pre-training has been shown to be beneficial across different branches of natural language processing. Unlike generative models that learn smooth manifolds \citep{kingma2013auto, goodfellow2014generative, rezende2015variational} for novel data generation, the model explicitly aims at learning powerful semantic representations that are beneficial for end tasks \citep{devlin2018bert, radford2018improving, liu2019roberta}.

In our work, we use the \textsc{BART} \citep{lewis2019bart} encoder-decoder model, trained using an auto-encoding denoising objective.  The model is trained by reconstructing input documents that were corrupted using a heuristic; such as word masking, word dropping, and sentence shuffling. Input corruption forces the decoder to rely on local and global dependencies to perform denoising, instead of only `copying' information from the input. Also, the configuration has a close alignment to the abstractive summarization setting. The decoder has to operate in two modes of `copying` directly from the input, leveraging the attention mechanism, and generating novel words \citep{see2017get}. The latter arguably requires a more sophisticated machinery that involves information aggregation, entailment, and paraphrasing. 

The model parameters $\theta$ are further fine-tuned on article-summary pairs $\{x_i, y_i\}_{i=1}^N$ by estimating a conditional model $p_{\theta}(y|x)$ in Eq. \ref{eq:fine-tuning-kld-mc} using Monte Carlo approximation.

% by maximizing their conditional probabilities in Eq. \ref{eq:abstr_obj}. 

% From the theoretical perspective, the aim is to estimate the conditional distribution that governs generation of summaries by minimizing Kullback-Leibler divergence in Eq. \ref{eq:kld}.

\begin{equation}
\begin{aligned}
     \theta^{*} =& \argmin_{\theta} \mathbb{E}_{x \sim p(x)}\left[\KL{p(y|x)}{p_{\theta}(y|x)} \right]\\=& 
 \argmax_{\theta} \mathbb{E}_{(x,y) \sim p(x,y)}\left[ \log p_{\theta}(y|x) \right] \\
 \approx& \argmax_{\theta} \dfrac{1}{N} \sum_{i=1}^N \log p_{\theta}(y_i|x_i) \\
 =& \argmax_{\theta} \mathcal{L}_{abs}(\theta)
   \label{eq:fine-tuning-kld-mc}
\end{aligned}
 \end{equation}

% \begin{equation}
%     \mathcal{L}_{abs}(\theta) = \sum_{i=1}^N \log p_{\theta}(y_i|x_i)
%     \label{eq:abstr_obj}
% \end{equation}

% This objective combined with annotated data allows to readjust the model parameters to be more specific towards abstractive summary generation. 

\subsection{Joint Models}
\label{sec:joint_model}

The conditional model $p_{\theta}(y|x)$ estimation is a prevalent modern approach. Following \citet{minka2005discriminative}, we show that it can be derived from a broader model by making a few modelling assumptions. We start with a joint model over both the input $x$ and output $y$, $p_{\theta, \hat{\theta}}(x, y) = p_{\theta}(y|x) p_{\hat{\theta}}(x)$, with two parameter sets $\theta$ and $\hat \theta$. The model, in turn, can be estimated as shown in Eq. \ref{eq:joint-kld}.

\begin{equation}
    \begin{aligned}
    \theta^{*}, \hat\theta^{*} =& \argmin_{\theta, \hat \theta} \KL{p(y,x)}{p_{\theta, \hat{\theta}}(x, y)} \\
     =&\argmax_{\theta, \hat \theta}  \mathbb{E}_{x \sim p(x)}\left[ \log p_{\hat \theta}(x) \right] + \\&\mathbb{E}_{(x,y) \sim p(x,y)}\left[ \log p_{\theta}(y|x) \right] 
     \label{eq:joint-kld}
\end{aligned}
\end{equation}


% \begin{equation}
%     p_{\theta, \hat{\theta}}(x, y) = p_{\theta}(y|x) p_{\hat{\theta}}(x) 
%     \label{eq:joint_model}
% \end{equation}

% Here, $p_{\hat{\theta}}(x)$ corresponds to the prior over input with parameters $\hat{\theta}$. 

By assuming $\hat \theta$ to be fixed or independent of $\theta$, for example, $p_{\hat{\theta}}(x)$ a uniform distribution over the support; the parameter search for $\theta^{*}$ becomes equivalent in Eqs. \ref{eq:fine-tuning-kld-mc} and \ref{eq:joint-kld}. In other words, the term related to $p_{\hat{\theta}}(x)$ can be safely ignored as it do not contribute to the gradient. 

However, $p_{\hat{\theta}}(x)$ can be useful in its own right. First of all, unlike $p_{\theta}(y|x)$, it does not require annotations $y$, which might not be readily available, such as in scarcely annotated domains or for transduction, as we dicuss next. Second, by parameters coupling, $\hat{\theta}$ = $\theta$, it's possible to leverage input statistical regularities to improve the predictive power of $p_{\theta}(y|x)$. For example, in news summarization, it's well known that summaries derived directly from input document fragments are hard to beat baselines \citep{nallapati2016summarunner, see2017get, liu2019text}. In this light, we hypothesized that explicit modelling of such fragments, with shared parameters, can steer the conditional model $p_{\theta}(y|x)$ towards generation of better summaries. 


\subsection{Transductive Learning}

The modern approach in machine learning is to learn a model that possesses generalization power to unseen data samples. 
% Some implicit assumptions about data are often made, such as training and test time data samples are identically distributed. 
This approach is known as \textit{inductive learning}, which, in essence, aims at learning an abstract set of rules governing the whole data distribution. On the other hand, \textit{transductive learning} \citep{vapnik1998statistical}, is a learning framework that aims at learning a set of abstract rules that govern a specific sample of data. In practice, we might not be interested in a model that is able to generate high quality summaries for an arbitrary sample of articles. Instead, our task might be more narrowly focused to a specific sample. Additionally, the articles might be different from the ones the model has seen in training. For example, we might train a model on a large corpus of news from 2007 to 2015, yet want to test on articles from 2017. 

We hypothesized that the joint formulation where the input is modelled explicitly, can be useful for the task of test set adaptation. Specifically, the model that is fine-tuned on the training set can benefit from a subsequent exposure to the input of the test set. Intuitively, the model can adapt to specifics in the input, such as new entities, actors, and event. And consequently, learn to produce higher quality summaries. 


==> summs/front_summ.tex <==
% \textcolor{red}
% \textcolor{orange}
% \textcolor{blue}
% \textcolor{cyan}
% \textcolor{myGreen}
% B009L0KU46

\begin{table}[t!]
    \centering
 	\footnotesize 
    \begin{tabular}{ >{\centering\arraybackslash} m{1.5cm} m{5cm}} 
 \thickhline
    \textbf{Abstractive} & \vspace{0.5em} \textcolor{orange}{A photo of a green woodpecker flying with a weasel on its back has gone viral on Twitter.} The image was snapped by amateur photographer Martin Le-May near London. It sparked the hashtag \#weaselpecker and has spawned numerous memes. \vspace{0.5em}  \\ \thickhline
    \textbf{Extractive} & \vspace{0.5em} \textcolor{orange}{A photo of a weasel hitching a surprise lift on the back of a flying woodpecker near London has gone viral on Twitter}, with more than 7,000 users retweeting the original post of the image. It was \textcolor{red}{first posted by photographer Jason Ward} on Monday and credited to Martin Le-May. \vspace{0.5em} 
\\ \thickhline
    \end{tabular}
    \caption{Example of a gold abstractive and extractive summary. Here the extractive summary contains a \textcolor{orange}{paraphrase} and a \textcolor{red}{complementary important fact}.}
    \label{table:front-example-summ}
\end{table}

